QoS aware Automatic Web Service Composition with Multiple objectives

With an increasing number of web services, providing an end-to-end Quality of Service (QoS) guarantee in responding to user queries is becoming an important concern. Multiple QoS parameters (e.g., response time, latency, throughput, reliability, availability, success rate) are associated with a service, thereby, service composition with a large number of candidate services is a challenging multi-objective optimization problem. In this paper, we study the multi-constrained multi-objective QoS aware web service composition problem and propose three different approaches to solve the same, one optimal, based on Pareto front construction and two other based on heuristically traversing the solution space. We compare the performance of the heuristics against the optimal, and show the effectiveness of our proposals over other classical approaches for the same problem setting, with experiments on WSC-2009 and ICEBE-2005 datasets.

==> Working_Example.tex <==
\section{Motivating Example}\label{sec:example}
\noindent
In this section, we explain the motivation of our work on a simple intuitive example. 
Consider the services defined in Table~\ref{tab1}.
The service dependency graph is shown in Figure \ref{Composition}. 
% The input-output dependencies of the services are shown in Figure \ref{Composition}. 
Consider a service query request with ${\cal{R}}_i = \{i_1, i_2, i_3\}$ with an objective to obtain
${\cal{R}}_o = \{o_{12}, o_{13}\}$ as response. 
% To resolve the given query request, a classical service composition method would produce a solution consisting of the
A desired solution for the query is the sequence of services to be composed to
arrive at the desired query output starting from the query inputs. Evidently, a number of solutions are possible
as discussed below, each having different QoS value for the composite solution.
Consider, for example, the solution ${\cal{Q}}_1 : S_1; S_4; [S_6 || S_7]$, 
where $S_1$, $S_4$ and the parallel combination $[S_6 || S_7]$ are executed sequentially 
($S_6$ and $S_7$ are executed in parallel). 
This solution has the best QoS in terms of the number of invoked services and the throughput as 30000.
In the solution ${\cal{Q}}_1$, the throughput is calculated as, min (50000, 30000, min (40000, 45000)) = 30000.
Considering response time as the primary objective, the best solution is achieved by 
 ${\cal{Q}}_2 : [S_1 || S_2 || S_3]; S_5; [S_7 || S_8]$, which has the minimum response time value as 800 ms.
In the solution ${\cal{Q}}_2$, $S_1, S_2, S_3$ are executed in parallel, $S_7, S_8$ are executed in parallel and the 
combination $[S_1 || S_2 || S_3]$, $S_5$ and the combination $[S_7 || S_8]$ are executed 
sequentially. Therefore, the response time is max(100, 150, 100) + 200 + max(400, 450) = 800ms.

\begin{table}[htb]
\scriptsize
\caption{\small{Definition of services}}
 \begin{center}
  \begin{tabular}{|c|c|c|c|c|}
   \hline
   \textbf{Service} & \textbf{Input} & \textbf{Output} & \textbf{RT(ms)} & \textbf{TR}\\
   \hline
   \hline
   $S_1$ & $\{i_1\}$ & $\{i\-o_4, i\-o_5\}$ & 100 & 50000\\
   \hline
   $S_2$ & $\{i_2\}$ & $\{i\-o_6\}$ & 150 & 45000\\
   \hline
   $S_3$ & $\{i_3\}$ & $\{i\-o_7\}$ & 100 & 10000\\
   \hline
   $S_4$ & $\{i\-o_4\}$ & $\{i\-o_8, i\-o_9\}$ & 250 & 30000\\
   \hline
   $S_5$ & $\{i\-o_5, i\-o_6, i\-o_7\}$ & $\{i\-o_9, i\-o_{10}, i\-o_{11}\}$ & 200 & 10000\\
   \hline
   $S_6$ & $\{i\-o_8, i\-o_9\}$ & $\{o_{12}\}$ & 500 & 40000\\
   \hline
   $S_7$ & $\{i\-o_9\}$ & $\{o_{13}\}$ & 400 & 45000\\
   \hline
   $S_8$ & $\{i\-o_{10}\}$ & $\{o_{12}\}$ & 450 & 40000\\
   \hline
   $S_9$ & $\{i\-o_{11}\}$ & $\{o_{13}\}$ & 550 & 50000\\
   \hline
  \end{tabular}
 \end{center}\label{tab1}
\end{table}
\begin{figure}[!ht]
\centering
\includegraphics[height=2.5cm,width=5cm]{fig/2.pdf}
\caption{Service dependency graph}
\label{Composition}
\end{figure}

\noindent
An obvious solution for optimal Q0S-based composition is to explore all paths (or possible sub graphs) 
of the dependency graph (Figure \ref{Composition}),
calculate the values of the QoS parameters for each possibility and choose the path (or subgraph) which has the best QoS. 
If different QoS parameters give different solution, we can choose the solution which has the best QoS value 
for one of the parameters and the values for the rest of the parameters as good as possible.
Evidently the solution may not be unique and may vary depending on the choice of the parameter taken as the primary objective.
We first consider {\em response time} as the primary QoS parameter.
\cite{6649580} proposed an iterative solution, where using a forward QoS computation technique, 
for each node ${\cal{N}}_i$ of the dependency graph, 
the best response time for the composition solutions till the node ${\cal{N}}_i$ is calculated.
% Finally, the best solution is chosen from the node(s) which produce(s) the requester's desired output.
Following this construction, we get ${\cal{Q}}_2$ as the solution for the above example.
On the other hand, if we consider {\em throughput} as the primary QoS parameter,
following the same construction, we get ${\cal{Q}}_1$ as the optimal solution for the above example.
If we consider both simultaneously, the answer is not obvious. Finding the optimal solution considering multiple QoS parameters is a nontrivial challenge, and we address this in this paper.
% Moreover, the best QoS solution construction method needs to be fast and scalable. 
\\

\noindent
{\textbf {Our contribution :}}
Contemporary approaches existing in literature take considerable time to produce the best solution at runtime.
In this proposal, on one hand, we use a single QoS aware path selection technique for resolving a given service query 
in a fast and efficient way.
This is a modest elaborate version of our contribution in \cite{chattopadhyay2015scalable}.
On the other hand, we additionally address the problem of multiple QoS parameters and propose a path selection strategy. 
The essential idea behind our approach is to 
% deterministically / probabilistically 
select and construct a 
query solution path beginning with the desired output and progressively traverse backward on the service dependency graph.
Though our scheme does not guarantee the best solution in terms of QoS, we show that we can achieve a close to optimal
solution in considerably less time than the contemporary approaches.
We also propose a parameterized search algorithm that improves on solution quality at the cost of computation time.
In the next section, we discuss the detailed methodology behind our proposals.
